Coding for Intelligence from the Perspective of Category

Coding, which targets compressing and reconstructing data, and intelligence, often regarded at an abstract computational level as being centered around model learning and prediction, interweave recently to give birth to a series of significant progress. The recent trends demonstrate the potential homogeneity of these two fields, especially when deep-learning models aid these two categories for better probability modeling. For better understanding and describing from a unified perspective, inspired by the basic generally recognized principles in cognitive psychology, we formulate a novel problem of Coding for Intelligence from the category theory view. Based on the three axioms: existence of ideal coding, existence of practical coding, and compactness promoting generalization, we derive a general framework to understand existing methodologies, namely that, coding captures the intrinsic relationships of objects as much as possible, while ignoring information irrelevant to downstream tasks. This framework helps identify the challenges and essential elements in solving the specific derived Minimal Description Length (MDL) optimization problem from a broader range, providing opportunities to build a more intelligent system for handling multiple tasks/applications with coding ideas/tools. Centering on those elements, we systematically review recent processes of towards optimizing the MDL problem in more comprehensive ways from data, model, and task perspectives, and reveal their impacts on the potential CfI technical routes. After that, we also present new technique paths to fulfill CfI and provide potential solutions with preliminary experimental evidence. Last, further directions and remaining issues are discussed as well. The discussion shows our theory can reveal many phenomena and insights about large foundation models, which mutually corroborate with recent practices in feature learning.

==> sources/abstract.tex <==
\begin{abstract}
%
Coding, which targets compressing and reconstructing data, and intelligence, \wh{often regarded at an abstract computational level as being centered around model learning and prediction}, interweave recently to give birth to a series of \wh{significant} progress.
The recent trends demonstrate the potential homogeneity of these two fields, especially when deep-learning models aid these two categories for better probability modeling.
%
For better understanding and describing from a unified perspective, we formulate a novel problem of \textit{Coding for Intelligence} from the category view, which provides a general framework to understand existing methodologies.
%
It helps identify the challenges and \wh{essential} elements in solving the related optimization problem from a broader range, providing opportunities to build a more intelligent system for handling multiple tasks/applications \wh{with coding ideas/tools}.
%
Centering on those elements, we systematically review recent processes of supporting techniques from data, model, and task perspectives, and reveal their potential impacts on the potential CfI technical routes.
%
After that, we also present new technique paths \wh{with the} potential to construct CfI architectures and provide potential solutions with preliminary experimental evidence.
Last, further direction is discussed as well.
%
% In this paper, we explore the new paradigm that connects these two fields, termed Coding for Intelligence (CfI), which optimizes the performance of an intelligent system constrained by data sample compression, data distribution compression, and data collection effort minimization,~\textit{etc}.
%
% We first formulate this optimization problem from the perspective of category theory, which gives a general form to construct an intelligent system with the help of compactness.
% %
% This general form is then specified and simplified into a linear form, consistent with the definition of Minimum Description Length (MDL), which considers the overview length of an intelligent system with the consideration of both performance and comprehensive costs in terms of data sample, data distribution, and data collection effort, \textit{etc}.
% %
% Then, we review the related diverse efforts in solving its variant sub-problems during different historical stages.
% %
% After that, from the formulation, we observe critical technical implications, \textit{e.g.} the joint model and representation compactness seldom paid attention to, which has the potential to further promote the intelligence.
% %
% Centering on those implications, we systematically review state-of-the-art techniques that support the related elements, 
% which provides the academic and industrial evidences to realize the collaborative optimization of the whole intelligent system via minimizing the proposed optimization function from a broader view.
% %
% Then, we come up with several potential CFI routes, and the preliminary results demonstrate the performance and efficiency gains in contributing CFI. 
% Last, further direction is discussed as well.
\end{abstract}

\begin{IEEEkeywords}
Coding for intelligence,
multi-task collaboration,
multi-modality coding,
artificial intelligence,
category theory
\end{IEEEkeywords}


==> sources/bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_image/Wenhan_Yang.png}}]
		{Wenhan Yang} (Member, IEEE)
		received the B.S. degree and Ph.D. degree (Hons.) in computer science from Peking University, Beijing, China, in 2012 and 2018.
        He is currently an associate researcher with PengCheng Laboratory, Shenzhen, Guangdong, China.
        His current research interests include image/video processing/restoration, bad weather restoration, and human-machine collaborative coding.
        %
        He has authored over 50 technical articles in refereed journals and proceedings, and holds 9 granted patents. He received the 2023 IEEE Multimedia Rising Star Runner-Up Award, the IEEE ICME-2020 Best Paper Award, the IFTC 2017 Best Paper Award, the IEEE CVPR-2018 UG2 Challenge First Runner-up Award, and the MSA-TC Best Paper Award of ISCAS 2022. He was the Candidate of CSIG Best Doctoral Dissertation Award in 2019.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_image/Zixuan_Hu.jpg}}]
		{Zixuan Hu} (Graduate Student Member, IEEE) received his B.S. degree at the School of Mathematical Sciences, Peking University, Beijing, China, in 2023. He is currently pursuing his Ph.D. degree at the School of Computer Science, Peking University. His current research interests include test-time adaptation, model selection, and machine learning algorithms. He has published several papers in prestigious conferences and journals such as CVPR, ICCV, and ECCV.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_image/linlilang.png}}]
		{Lilang Lin}(Student Member, IEEE) received the B.S. degree in data science from Peking University, Beijing, China, in 2021, where he is currently pursuing the Ph.D. degree with the Wangxuan Institute of Computer Technology. His current research interests include action recognition, self-supervised learning, and unsupervised learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_image/Jiaying_Liu.jpg}}]
		{Jiaying Liu} (Senior Member, IEEE)
		received the PhD degree (Hons.) in computer science from Peking University, Beijing China, 2010. She is currently an Associate Professor, Boya Young Fellow with the Wangxuan Institute of Computer Technology, Peking University, China. She has authored more than 100 technical articles in refereed journals and proceedings, and holds 70 granted patents. Her current research interests include multimedia signal processing, compression, and computer vision. She is a senior member of IEEE/CSIG, and a distinguished member of CCF. She was a visiting scholar with the University of Southern California, Los Angeles, California, from 2007 to 2008. She was a visiting researcher with Microsoft Research Asia, in 2015 supported by the Star Track Young Faculties Award.
		
		Dr. Liu has served as a member of Multimedia Systems and Applications Technical Committee (MSA TC), and Visual Signal Processing and Communications Technical Committee (VSPC TC) in IEEE Circuits and Systems Society. She received the IEEE ICME 2020 Best Paper Award and IEEE MMSP 2015 Top10\% Paper Award.
		%
		She has also served as the Associate Editor of the IEEE Trans. on Image Processing, the IEEE Trans. on Circuits Systems for Video Technology and Journal of Visual Communication and Image Representation, the Technical Program Chair of ACM MM Asia-2023/IEEE ICME-2021/ACM ICMR-2021/IEEE VCIP-2019, the Area Chair of CVPR-2021/ECCV-2020/ICCV-2019, ACM ICMR Steering Committee member and the CAS Representative at the ICME Steering Committee. She was the APSIPA Distinguished Lecturer (2016-2017).
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio_image/Ling-Yu_Duan.jpg}}]
		{Ling-Yu Duan} is a Full Professor with the National Engineering Laboratory of Video Technology (NELVT), School of Electronics Engineering and Computer Science, Peking University (PKU), China, and has served as the Associate Director of the Rapid-Rich Object Search Laboratory (ROSE), a joint lab between Nanyang Technological University (NTU), Singapore, and Peking University (PKU), China since 2012. He is also with Peng Cheng Laboratory, Shenzhen, China, since 2019. He received the Ph.D. degree in information technology from The University of Newcastle, Callaghan, Australia, in 2008. His research interests include multimedia indexing, search, and retrieval, mobile visual search, visual feature coding, and video analytics, etc. He has published about 200 research papers. He received the IEEE ICME Best Paper Award in 2019/2020, the IEEE VCIP Best Paper Award in 2019, and EURASIP Journal on Image and Video Processing Best Paper Award in 2015, the Ministry of Education Technology Invention Award (First Prize) in 2016, the National Technology Invention Award (Second Prize) in 2017, China Patent Award for Excellence (2017), the National Information Technology Standardization Technical Committee "Standardization Work Outstanding Person" Award in 2015. He was a Co-Editor of MPEG Compact Descriptor for Visual Search (CDVS) Standard (ISO/IEC 15938-13) and MPEG Compact Descriptor for Video Analytics (CDVA) standard (ISO/IEC 15938-15). Currently he is an Associate Editor of IEEE Transactions on Multimedia, ACM Transactions on Intelligent Systems and Technology and ACM Transactions on Multimedia Computing, Communications, and Applications, and serves as the area chairs of ACM MM and IEEE ICME. He is a member of the MSA Technical Committee in IEEE-CAS Society. 
\end{IEEEbiography}


